NESC: Robust Neural End-2-End Speech Coding with GANs

Neural networks have proven to be a formidable tool to tackle the problem of speech coding at very low bit rates. However, the design of a neural coder that can be operated robustly under real-world conditions remains a major challenge. Therefore, we present Neural End-2-End Speech Codec (NESC) a robust, scalable end-to-end neural speech codec for high-quality wideband speech coding at 3 kbps. The encoder uses a new architecture configuration, which relies on our proposed Dual-PathConvRNN (DPCRNN) layer, while the decoder architecture is based on our previous work Streamwise-StyleMelGAN. Our subjective listening tests on clean and noisy speech show that NESC is particularly robust to unseen conditions and signal perturbations.

==> IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> sections/related_work.tex <==
\section{Related Work}
\label{sec:related_work}

For a comprehensive list of existing work on post-filtering with neural networks we refer to~\cite{postgan}.
The first work to show the feasibility of low bit rate neural speech coding was~\cite{wavenet_coding}, using a fairly complex WaveNet decoder.
The complexity issue was partially tackled with a different approach in~\cite{samplernn_coding}.

\improve{add more level 1 papers}.

The \ac{lpcnet} model~\cite{lpcnet_coding} was the first to enable neural speech coding of clean speech able to run on edge devices.
Its decoder is an autoregressive architecture based on WaveRNN, which is aggressively pruned to use only a fraction of its initial weights, so that the resulting model is low in complexity.
\ac{lpcnet} has a very low bit rate of \kbps{1.6}, and its coding parameters include the Bark-scale cepstrum, the pitch information and the energy.
Our previously presented model~\cite{ssmgan} is also able to decode this same bitstream, while achieving higher quality synthesis with moderate complexity and more parallelization potential.

The more recent work~\cite{lyra} presented \ac{lyra}, a new neural speech decoder compressing speech at \kbps{3}.
The encoder directly codes stacked mel-spectra and the decoder uses noise suppression and variance regularization to improve the quality of out-of-distribution samples.
\ac{lyra} was the first model specifically designed to work under more general conditions, e.g. for noisy speech.

The work~\cite{sstream} introduced \ac{sstream}, the first level 3 neural codec able to robustly code signals at very low bit rates, ranging from \kbps{3} to \kbps{12}.
\ac{sstream} is robust against noise and reverberation, can code music, and offers the possibility to perform noise reduction.
The complexity of its encoder and decoder architecture are both in the order of magnitude of \ac{ssmgan}'s decoder, hence making optimizations for deployment on edge devices foreseeable.
Very recently the work~\cite{tfnet} appeared also claiming to be able to do robust high quality speech coding at \kbps{3}.

\improve{add Kim's papers and explain that they target other bit-rates}


